Minimal Schedule with Minimal Number of Agents in Attack-Defence Trees

Expressing attack-defence trees in a multi-agent setting allows for studying a new aspect of security scenarios, namely how the number of agents and their task assignment impact the performance, e.g. attack time, of strategies executed by opposing coalitions. Optimal scheduling of agents' actions, a non-trivial problem, is thus vital. We discuss associated caveats and propose an algorithm that synthesises such an assignment, targeting minimal attack time and using minimal number of agents for a given attack-defence tree.

==> examples/tabAttributes_forestall.tex <==
%!TEX root=./report_IEEE.tex

\begin{tabular}{l@{$\,:\;$}l@{~}l@{~}r}
	\multicolumn{2}{l}{\textbf{Name}} & \textbf{Cost} & \textbf{Time}\\
	\hline
	\gate{FS}  & forestalling of softw. & \EUR{0}   & 10~d\\
	\gate{SC}  & steal code             & \EUR{0}   &  0~d\\
	\gate{PRS} & physical robbery succ. & \EUR{0}   &  0~d\\
	\gate{PR}  & physical robbery       & \EUR{0}   &  0~d\\
	\gate{NAS} & network attack succ.   & \EUR{0}   &  0~d\\
	\gate{NA}  & network attack         & \EUR{0}   &  1~d\\
	\gate{BRB} & bribe                  & \EUR{0}   &  3~d\\
	\leaf{icp} & integr.\ code in prod. & \EUR{2k}  & 15~d\\
	\leaf{dtm} & deploy to market       & \EUR{1k}  &  5~d\\
	\leaf{scr} & secure coding rooms    & \EUR{5k}  &  0~d\\
	\leaf{rfc} & rob.\ finds code       & \EUR{0}   &  0~d\\
	\leaf{reb} & rob.\ enters building  & \EUR{500} &  3~d\\
	\leaf{hr}  & hire robber            & \EUR{4k}  & 10~d\\
	\leaf{id}  & intrusion detection   & \EUR{200} &  1~d\\
	\leaf{heb} & hacker exploits bug    & \EUR{0}   &  3~d\\
	\leaf{sb}  & system has a bug       & \EUR{0}   &  0~d\\
	\leaf{hh}  & hire hacker            & \EUR{1k}  & 20~d\\
	\leaf{psc} & progr.\ steals code    & \EUR{0}   &  7~d\\
	\leaf{bp}  & bribe programmer       & \EUR{2k}  & 15~d\\
\end{tabular}


==> examples/tabAttributes_gainadmin.tex <==
%!TEX root=./report_IEEE.tex

\begin{tabular}{l@{$\,:\;$}l@{~}l@{~}r}
	\multicolumn{2}{l}{\textbf{Name}} & \textbf{Cost} & \textbf{Time}\\
	\hline
	\gate{OAP}  & obtain admin privileges & \EUR{0}   &  0~m\\
	\gate{GSAP} & get SA password         & \EUR{0}   &  0~m\\
	\gate{ACLI} & access c.c.\ CLI        & \EUR{0}   &  2~m\\
	\gate{TSA}  & trojan horse for SA     & \EUR{0}   &  0~m\\
	\gate{DTH}  & defence against trojans & \EUR{0}   &  0~m\\
	\gate{LSAS} & LSA successful          & \EUR{0}   &  0~m\\
	\gate{LSA}  & look over SA shoulder   & \EUR{0}   &  0~m\\
	\gate{GAPS} & GAP successful          & \EUR{0}   &  2~m\\
	\gate{GAP}  & get admin password      & \EUR{0}   & 10~m\\
	\gate{ECCS} & enter c.c.\ successful  & \EUR{0}   &  1~h\\
	\gate{ECC}  & enter computer centre   & \EUR{0}   &  0~d\\
	\leaf{csa}  & corrupt Sys.\ Admin.    & \EUR{5k}  &  5~d\\
	\leaf{efw}  & E-Mail firewall         & \EUR{3k}  &  0~m\\
	\leaf{wd}   & watchdog sys.\ daemon   & \EUR{2k}  &  5~m\\
	\leaf{th}   & trojan horse SA         & \EUR{100} &  3~d\\
	\leaf{nv}   & no-visits policy        & \EUR{0}   &  0~d\\
	\leaf{sat}  & spy SA terminal         & \EUR{0}   & 30~m\\
	\leaf{vsa}  & visit SA at work        & \EUR{20}  &  2~d\\
	\leaf{bsa}  & befriend Sys.\ Admin.   & \EUR{500} & 14~d\\
	\leaf{tla}  & two-level authentic.    & \EUR{5}   &  1~m\\
	\leaf{fgp}  & find guessable pass.   & \EUR{0}   &  1~d\\
	\leaf{opf}  & obtain password file    & \EUR{100} &  3~d\\
	\leaf{scr}  & secure coding rooms     & \EUR{5k}  &  0~d\\
	\leaf{ccg}  & c.c.\ guest unwatched   & \EUR{100} &  5~d\\
	\leaf{bcc}  & break-in comp.\ centre  & \EUR{6k}  &  2~d\\
	\leaf{co}   & corrupt operator        & \EUR{4k}  &  4~d\\
\end{tabular}


==> examples/tabAttributes_interrupted.tex <==
%!TEX root=../main.tex

\begin{tabular}{l@{~}r}
	\textbf{Name} & \textbf{Time}\\
	\hline
	\leaf{a} &  0~m\\
	\leaf{b} &  2~m\\
	\leaf{c} &  1~m\\
	\leaf{d} &  4~m\\
	\leaf{e} &  3~m\\
\end{tabular}


==> examples/tabAttributes_iotdev.tex <==
%!TEX root=./report_IEEE.tex

\begin{tabular}{l@{$\,:\;$}l@{~}l@{~}r}
	\multicolumn{2}{l}{\textbf{Name}} & \textbf{Cost} & \textbf{Time}\\
	\hline
	\gate{CIoTD} & compromise IoT device    & \EUR{0}   &  0~h\\
	\gate{APNS}  & access private net.\ succ. & \EUR{0} &  1~m\\
	\gate{APN}   & access private net.      & \EUR{0}   &  3~m\\
	\gate{GVC}   & get valid credentials    & \EUR{0}   &  0~h\\
	\gate{CPN}   & connect to private net.  & \EUR{0}   &  0~h\\
	\gate{AW}    & access WLAN              & \EUR{0}   &  0~h\\
	\gate{AL}    & access LAN               & \EUR{0}   &  0~h\\
	\leaf{rms}   & run malicious script     & \EUR{100} & 30~m\\
	\leaf{esv}   & exploit soft.\ vulnerab. & \EUR{10}  &  1~h\\
	\leaf{inc}   & inform of new connect.   & \EUR{5}   &  1~m\\
	\leaf{tla}   & two-level authentic.     & \EUR{5}   &  1~m\\
	\leaf{gc}    & get credentials          & \EUR{100} & 10~h\\
	\leaf{bwk}   & break WPA keys           & \EUR{100} &  2~h\\
	\leaf{fw}    & find WLAN                & \EUR{10}  &  5~h\\
	\leaf{sma}   & spoof MAC address        & \EUR{50}  & 30~m\\
	\leaf{flp}   & find LAN port            & \EUR{10}  &  1~h\\
\end{tabular}


==> examples/tabAttributes_last.tex <==
%!TEX root=../main.tex

\begin{tabular}{l@{~}r}
	\textbf{Name} & \textbf{Time}\\
	\hline
	\leaf{a} &  0~m\\
	\leaf{b} &  1~m\\
	\leaf{c} &  1~m\\
	\leaf{d} &  3~m\\
	\leaf{e} &  0~m\\
	\leaf{f} &  0~m\\
	\leaf{g} &  0~m\\
	\leaf{h} &  0~m\\
	\leaf{i} &  0~m\\
	\leaf{j} &  1~m\\
	\leaf{k} &  0~m\\
	\leaf{l} &  1~m\\
	\leaf{m} &  0~m\\
\end{tabular}


==> examples/tabAttributes_scaling.tex <==
%!TEX root=../main.tex

\begin{tabular}{l@{~}r}
	\textbf{Name} & \textbf{Time}\\
	\hline
	\leaf{a} &  1~m\\
	\leaf{b} &  1~m\\
	\leaf{c} &  1~m\\
	\leaf{d} &  1~m\\
	\leaf{e} &  3~m\\
	\leaf{f} &  1~m\\
	\leaf{g} &  1~m\\
\end{tabular}


==> examples/tabAttributes_toy_example.tex <==
%!TEX root=../main.tex

\begin{tabular}{l@{~}r}
	\textbf{Name} & \textbf{Time}\\
	\hline
	\gate{A7} &  1~m\\
	\gate{A6} &  1~m\\
	\gate{A5} &  1~m\\
	\gate{A4} &  1~m\\
	\gate{A3} &  1~m\\
	\gate{A2} &  1~m\\
	\gate{A1} &  1~m\\
	\leaf{l8} &  1~m\\
	\leaf{l7} &  1~m\\
	\leaf{l6} &  1~m\\
	\leaf{l5} &  1~m\\
	\leaf{l4} &  1~m\\
	\leaf{l3} &  1~m\\
	\leaf{l2} &  1~m\\
	\leaf{l1} &  1~m\\
\end{tabular}


==> related.tex <==
%!TEX root=./main.tex

\paragraph*{Related work}
% \label{sec:intro:relatedwork}

\ADT/s \cite{KordyMRS10,KMRS14}
are a popular formalism that has been implemented in a broad range
of analysis frameworks \cite{Gadyatskaya_2016,AGKS15,GIM15,ANP16},
comprehensively surveyed in \cite{KPCS13,WAFP19}.
They remain extensively studied today \cite{FilaW20}.
Of particular relevance is the \ADT/ to AMAS translation \cite{ICFEM2020},
based on the semantics from \cite{AAMASWJWPPDAM2018a}.
Furthermore, the problem discussed in this paper is clearly related to
parallel program scheduling \cite{CompSched,KwokA99}.
%According to literature \cite{CompSched,KwokA99},
%scheduling algorithms for Task Precedence Graphs can be divided both depending on the structure of a scheduled graph and on a number of available resources (processors).
%and can be classified either as a Unit Computational Cost (UCC) or a No Communication (NC) graph scheduling problem.
Due to time normalisation, it falls into the category of Unit Computational Cost (UCC) graph scheduling problems,
which can be effectively solved for tree-like structures \cite{Hu1961},
but cannot be directly applied to a set of \DAG/s.
Although a polynomial solution for interval-ordered \DAG/s was proposed by \cite{PapaYan1979},
their algorithm does not guarantee the minimal number of agents.
%
Due to zero-cost communication in all considered graphs, the problem can also be classified as No Communication (NC) graph scheduling.
A number of heuristic algorithms using list scheduling were proposed \cite{CompSched}, including
Highest Levels First with No Estimated Times (HLFNET),
Smallest Co-levels First with no Estimated Times (SCFNET),
and Random, where nodes in the DAG are assigned priorities randomly.
Variants assuming non-uniform node computation times are also considered, 
but are not applicable to the problem solved in this paper.
Furthermore, this class of algorithms does not aim at finding a schedule with the minimal number of processors or agents.
%
On the other hand, known algorithms that include such a limit, \ie for the Bounded Number of Processors (BNP) class of problems,
assume non-zero communication cost and rely on the clustering technique,
reducing communication, and thus schedule length, by mapping nodes to processing units.
Hence, these techniques are not directly applicable. %here.

%Under the assumption that the co-level from the SCFNET heuristic corresponds to a proposed level of a node and the level from HLFNET heuristics is actually the depth of a node,
The algorithm described in this paper can be classified as list scheduling with a fusion of HLFNET and SCFNET heuristics,
but with additional restriction on the number of agents used.
The length of a schedule is determined as the length of the critical path of a graph.
The number of minimal agents needed for the schedule is found with bisection.

Branching schedules analogous to the variants induced by \gateOR and defence nodes have been previously explored,
albeit using different models that either include probability \cite{Towsley86}
or require an additional \DAG/ to store possible executions \cite{ElRewiniA95}.
Zero duration nodes are also unique to the \ADT/ setting.

To the best of our knowledge, this is the first work dealing with agents in this context.
Rather, scheduling in multi-agent systems typically focuses on agents' \textit{choices}
in cooperative or competitive scenarios, \eg in models such as BDI \cite{NunesL14,DannT0L20}.

%\lm{
%\paragraph{Comparison with other scheduling algorithms}
%
%According to literature \cite{CompSched,KwokA99}, scheduling algorithms for Task Precedence Graphs can be divided both depending on the structure of a scheduled graph and on a number of available resources (processors). Due to the graph structure, the problem discussed in this paper can be classified as a Unit Computational Cost (UCC) graph scheduling problem or as a No Communication (NC) graph problem.
%
%The resulting graph consists of nodes with unitary cost, therefore it falls into the UCC class of problems. Work of Hu \cite{Hu1961} shows, that such problems can be effectively solved for tree-like structures, therefore such a solution cannot be directly applied to the considered problem. In \cite{PapaYan1979}, Papadimitriou and Yannakakis proposed a polynomial solution for Interval-Ordered Directed Acyclic Graphs (DAG). This algorithm could be applied to the scheduled graph but it does not guarantee the minimal number of agents used.
%
%Since all the communication in this graph has cost of 0, solutions for NC graphs can be applied. For graphs with no communication and unit node cost a number of heuristic algorithms using list scheduling were proposed \cite{CompSched}:
%\begin{itemize}
 %\item Highest Levels First with No Estimated Times (HLFNET), in which level is the sum of computation costs of all the nodes along the longest path from the node to an exit node and all nodes are scheduled as if they were of unit cost,
 %\item Smallest Co-levels First with no Estimated Times (SCFNET), where nodes are considered according to their co-levels determined by computing the sum of the longest path from an entry node to the node and nodes are scheduled as if they were of unit costs,
 %\item Random, where nodes in the DAG are assigned priorities randomly.
%\end{itemize}
%For all these heuristics, the variants assuming non-uniform nodes computation times are also considered -- yet, they are not applicable to the problem solved in this paper. The algorithms from this class also do not aim at finding the minimal number of processors (agents) for a schedule.
%
%The limit on the number of agents can be determined by imposing a constraint being their limit and determining a schedule for so limited number of resources. The known algorithms for Bounded Number of Processors (BNP) class of problems assume non-zero communication cost and rely on the clustering technique, in which nodes are mapped to the same procesing unit to reduce communication and total graph schedule length. Since the in problem solved in this paper all the communication in the graph has zero cost, such techniques are not directly applicable here.
%
%Under the assumption, that the co-level from the SCFNET heuristic corresponds to a proposed level of a node and the level from HLFNET heuristics is actually the depth of a node, the algorithm described in this paper can be classified as a list scheduling algorithm with a fusion of HLFNET and SCFNET heuristics but with additional restriction on the number of agents used. The length of a schedule is determined as the length of a critical path of a graph. The number of minimal agents needed for the schedule is found with bisection.}
